MATHSENSEI: A Tool-Augmented Large Language Model for Mathematical Reasoning

Tool-augmented Large Language Models (TALMs) are known to enhance the skillset of large language models (LLMs), thereby, leading to their improved reasoning abilities across many tasks. While, TALMs have been successfully employed in different question-answering benchmarks, their efficacy on complex mathematical reasoning benchmarks, and the potential complementary benefits offered by tools for knowledge retrieval and mathematical equation solving are open research questions. In this work, we present MathSensei, a tool-augmented large language model for mathematical reasoning. We study the complementary benefits of the tools - knowledge retriever (Bing Web Search), program generator + executor (Python), and symbolic equation solver (Wolfram-Alpha API) through evaluations on mathematical reasoning datasets. We perform exhaustive ablations on MATH, a popular dataset for evaluating mathematical reasoning on diverse mathematical disciplines. We also conduct experiments involving well-known tool planners to study the impact of tool sequencing on the model performance. MathSensei achieves 13.5% better accuracy over gpt-3.5-turbo with Chain-of-Thought on the MATH dataset. We further observe that TALMs are not as effective for simpler math word problems (in GSM-8K), and the benefit increases as the complexity and required knowledge increases (progressively over AQuA, MMLU-Math, and higher level complex questions in MATH). The code and data are available at https://github.com/Debrup-61/MathSensei.

==> editable_draw_iofiles/Bing_module <==
<mxfile host="app.diagrams.net" modified="2023-11-28T06:51:06.140Z" agent="Mozilla/5.0 (Macintosh; Intel Mac OS X 10.15; rv:109.0) Gecko/20100101 Firefox/119.0" etag="YwvUOTWXedMO-_a_5wQb" version="22.1.4" type="google">
  <diagram name="Page-1" id="yosZnwvtYeACwBmyeTCc">
    <mxGraphModel grid="1" page="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" pageScale="1" pageWidth="850" pageHeight="1100" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="HmoVr-3HVrakVy1XK3cQ-5" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-2">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="240" y="370" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ifNo40p1RAdDYsW6pUvs-2" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-2" target="CBzDvX9ltago5Vxs7Bon-6">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-2" value="&lt;font color=&quot;#3333ff&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;br class=&quot;Apple-interchange-newline&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font color=&quot;#3333ff&quot; style=&quot;font-size: 16px;&quot;&gt;Determine the coordinates of the point \(P\) on the line \(y = -x + 6\) such that \(P\) is equidistant from the points \(A(10, -10)\) and \(O(0, 0)\)&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font color=&quot;#3333ff&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font color=&quot;#3333ff&quot; style=&quot;font-size: 16px;&quot;&gt;(that is, so that \(PA=PO\)). Express your answer as an ordered pair \((a, b)\).&lt;/font&gt;&lt;/div&gt;&lt;font color=&quot;#3333ff&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" vertex="1" parent="1">
          <mxGeometry x="490" y="170" width="330" height="170" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-4" value="&lt;font size=&quot;1&quot;&gt;&lt;b style=&quot;font-size: 15px;&quot;&gt;QUESTION&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="620" y="130" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ifNo40p1RAdDYsW6pUvs-7" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;entryX=0.687;entryY=-0.008;entryDx=0;entryDy=0;entryPerimeter=0;" edge="1" parent="1" target="CBzDvX9ltago5Vxs7Bon-10">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="940" y="520" as="sourcePoint" />
            <mxPoint x="788.5" y="695" as="targetPoint" />
            <Array as="points">
              <mxPoint x="820" y="520" />
              <mxPoint x="787" y="521" />
            </Array>
          </mxGeometry>
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-6" value="&lt;div&gt;&lt;font style=&quot;font-size: 17px;&quot;&gt;1. &lt;font color=&quot;#009900&quot;&gt;If we draw the foot of the perpendicular from the point to the line and any other segment joining the point to the line, we get a right triangle.&amp;nbsp;&lt;/font&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 17px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 17px;&quot;&gt;2. &lt;font color=&quot;#6666ff&quot;&gt;However, the second line segment drawn here will always be the hypotenuse of the right triangle formed.&lt;/font&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 17px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 17px;&quot;&gt;&amp;nbsp;3. &lt;font color=&quot;#9933ff&quot;&gt;The length of each line segment connecting the point and the line differs, but by definition the distance between point and line is the length of the line segment that is perpendicular to \\ (L\\). In other words, it is the shortest distance between them.&lt;br&gt;&lt;/font&gt;&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#fff2cc;strokeColor=#d6b656;" vertex="1" parent="1">
          <mxGeometry x="940" y="330" width="490" height="290" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-7" value="&lt;font style=&quot;font-size: 15px;&quot;&gt;&lt;b&gt;CONCEPTS SEARCH USING BING&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="1060" y="290" width="270" height="30" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-9" value="&lt;font style=&quot;font-size: 15px;&quot;&gt;&lt;b&gt;FINAL BING MODULE OUTPUT&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="530" y="1010" width="240" height="30" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-10" value="&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot; color=&quot;#009900&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot; color=&quot;#009900&quot;&gt;We can use the distance formula to set up an equation for the distance &lt;br&gt;between point $P(x,y)$ and each of the other two points, and then set those distances equal to each other.&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot; color=&quot;#9933ff&quot;&gt;Solving for $x$ and $y$, we get the coordinates of point $P$.To&lt;br&gt; find the point $P$ on the line $y=-x+6$ equidistant from the points &lt;br&gt;$A(10,-10)$ and $O(0,0)$, we need to find the perpendicular bisector of &lt;br&gt;the line segment connecting $A$ and $O$.&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot; color=&quot;#3333ff&quot;&gt;This will be the line that&amp;nbsp; passes through the midpoint of $AO$ and is perpendicular to $AO$. We can then find the intersection of this line with the line $y=-x+6$ to get the coordinates of $P$. The distance between $P$ and $A$ (or $O$) will be the same, and we can use the distance formula to find this distance &lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;strokeColor=#666666;fontColor=#333333;" vertex="1" parent="1">
          <mxGeometry x="360" y="630" width="530" height="370" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-15" value="&lt;div style=&quot;font-size: 15px;&quot;&gt;&lt;font style=&quot;font-size: 15px;&quot;&gt;&lt;b&gt;SIMILAR QUESTION SEARCH&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 15px;&quot;&gt;&lt;font style=&quot;font-size: 15px;&quot;&gt;&lt;b&gt;USING BING API&lt;br&gt;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="250" y="270" width="230" height="50" as="geometry" />
        </mxCell>
        <mxCell id="ifNo40p1RAdDYsW6pUvs-9" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;entryX=0.455;entryY=-0.024;entryDx=0;entryDy=0;entryPerimeter=0;" edge="1" parent="1" target="CBzDvX9ltago5Vxs7Bon-10">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="414.07000000000016" y="460" as="sourcePoint" />
            <mxPoint x="641.8000000000002" y="601.6400000000001" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="ifNo40p1RAdDYsW6pUvs-1" value="&lt;div&gt;&lt;font color=&quot;#660000&quot; style=&quot;font-size: 16px;&quot;&gt;Determine the coordinates of the point P on the line y=-x+6 such that P is equidistant from the points A (10,-10) and O (0,0) (that is, so that PA=PO). Express your answer as an ordered pair (a,b).&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font color=&quot;#660000&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font color=&quot;#660000&quot; style=&quot;font-size: 16px;&quot;&gt;Guest Mar 12, 2019 2 Answers #1 +1 Answer is (8,-2) Guest Mar 12, 2019 #2 +125689 +1&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font color=&quot;#660000&quot; style=&quot;font-size: 16px;&quot;&gt;&amp;nbsp;Let P = ( x, -x + 6) = (x, 6 - x) We want to solve this&quot;,&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font color=&quot;#660000&quot; style=&quot;font-size: 16px;&quot;&gt;Solution Verified by Toppr&lt;/font&gt;&lt;/div&gt; " style="shape=parallelogram;perimeter=parallelogramPerimeter;whiteSpace=wrap;html=1;fixedSize=1;fillColor=#ffe6cc;strokeColor=#d79b00;size=10;" vertex="1" parent="1">
          <mxGeometry x="-30" y="380" width="450" height="220" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> editable_draw_iofiles/Refine_error <==
<mxfile host="app.diagrams.net" modified="2023-11-27T08:47:32.064Z" agent="Mozilla/5.0 (Macintosh; Intel Mac OS X 10.15; rv:109.0) Gecko/20100101 Firefox/119.0" etag="8k_CcRq7FodsiCShMiUJ" version="22.1.4" type="google">
  <diagram name="Page-1" id="yosZnwvtYeACwBmyeTCc">
    <mxGraphModel grid="1" page="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" pageScale="1" pageWidth="850" pageHeight="1100" math="0" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="CBzDvX9ltago5Vxs7Bon-2" value="&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;from sympy import *&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;x = symbols(&#39;x&#39;)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;eq = Eq(x**4 + 5*x**3 + 9*x**2 - x - 14, 0)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Equation:\&quot;, eq)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;roots = solve(eq, x)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;integer_roots = [r for r in roots if r.is_integer()]&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Integer roots:\&quot;, integer_roots)&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" vertex="1" parent="1">
          <mxGeometry x="30" y="190" width="356.25" height="210" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-3" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;&#39;bool&#39; object is not callable&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f8cecc;strokeColor=#b85450;" vertex="1" parent="1">
          <mxGeometry x="98.13" y="440" width="181.87" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-4" value="&lt;b&gt;ORIGINAL&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="160" y="160" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-5" value="&lt;b&gt;ERROR&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="160" y="540" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-6" value="&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;from sympy import *&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;x = symbols(&#39;x&#39;)&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;eq = Eq(x**4 + 5*x**3 + 9*x**2 - x - 14, &lt;/font&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;0)&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Equation:\&quot;, eq)\&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;roots =solve(eq, x)&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;integer_roots = [r for r in roots if int(r) ==r]&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Integer roots:\&quot;, integer_roots)&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#fff2cc;strokeColor=#d6b656;" vertex="1" parent="1">
          <mxGeometry x="470" y="170" width="400" height="230" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-7" value="&lt;b&gt;REFINE ROUND1&lt;br&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="615" y="140" width="110" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-8" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;Cannot convert complex to int&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f8cecc;strokeColor=#b85450;" vertex="1" parent="1">
          <mxGeometry x="470.00000000000006" y="430" width="205.93" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-9" value="&lt;b&gt;ERROR&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="542.97" y="530" width="80" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-10" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;Changed &#39;is_integer()&#39; to &#39;int(r) == r&#39; to check if the roots are integers&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#d5e8d4;strokeColor=#82b366;" vertex="1" parent="1">
          <mxGeometry x="720" y="440" width="210" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-11" value="&lt;b&gt;ERRORS FIXED&lt;br&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="780" y="530" width="107.03" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-12" value="&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;from sympy import *&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;x = symbols(&#39;x&#39;) &lt;/font&gt;&lt;/div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;eq = Eq(x**4 + 5*x**3 + 9*x**2 - x - 14, 0)&lt;/font&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Equation:\&quot;, eq)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;roots =solve(eq, x)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;integer_roots = []&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;for r in roots:&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; if r.is_real and int(r) == r:&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp;&amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; &amp;nbsp; integer_roots.append(int(r))&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot; dir=&quot;ltr&quot;&gt;&lt;wbr&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;print(\&quot;Integer roots:\&quot;, integer_roots)&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#ffe6cc;strokeColor=#d79b00;" vertex="1" parent="1">
          <mxGeometry x="480" y="610" width="400" height="240" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-19" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-13" target="CBzDvX9ltago5Vxs7Bon-18">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-13" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;None&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f8cecc;strokeColor=#b85450;" vertex="1" parent="1">
          <mxGeometry x="480" y="910" width="170" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-14" value="&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Used the is_real() method to check if the roots are real.&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Fixed the incorrect way of checking if the roots are integers.&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#d5e8d4;strokeColor=#82b366;" vertex="1" parent="1">
          <mxGeometry x="690" y="910" width="260" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-15" value="&lt;b&gt;REFINE ROUND2&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="615" y="580" width="130" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-16" value="&lt;b&gt;ERROR&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="535" y="1000" width="80" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-17" value="&lt;b&gt;ERRORS FIXED&lt;br&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="760" y="1000" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-18" value="&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Equation: Eq(x**4 + 5*x**3 + 9*x**2 - x - 14, 0)&lt;/font&gt;&lt;/div&gt;&lt;div style=&quot;font-size: 16px;&quot;&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Integer roots: [-2, 1]&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" vertex="1" parent="1">
          <mxGeometry x="140" y="880" width="200" height="100" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-20" value="&lt;b&gt;FINAL PG OUTPUT&lt;br&gt;&lt;/b&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="180" y="980" width="130" height="10" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> editable_draw_iofiles/Walpha <==
<mxfile host="app.diagrams.net" modified="2023-11-28T03:18:42.646Z" agent="Mozilla/5.0 (Macintosh; Intel Mac OS X 10.15; rv:109.0) Gecko/20100101 Firefox/119.0" etag="Oi0_TdZ1deFtaSWeNX37" version="22.1.4" type="google">
  <diagram name="Page-1" id="yosZnwvtYeACwBmyeTCc">
    <mxGraphModel grid="1" page="1" gridSize="10" guides="1" tooltips="1" connect="1" arrows="1" fold="1" pageScale="1" pageWidth="850" pageHeight="1100" math="1" shadow="0">
      <root>
        <mxCell id="0" />
        <mxCell id="1" parent="0" />
        <mxCell id="ufljFMe3RaCTCH4WWNqV-2" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-2">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="550" y="260" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-2" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;Find the dot product of \[&lt;br&gt;\begin{pmatrix}&lt;br&gt;    -2 \\&lt;br&gt;    0 \\&lt;br&gt;    7&lt;br&gt;\end{pmatrix}&lt;br&gt;\quad \text{and} \quad&lt;br&gt;\begin{pmatrix}&lt;br&gt;    3 \\&lt;br&gt;    4 \\&lt;br&gt;    -5&lt;br&gt;\end{pmatrix}.&lt;br&gt;\]&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#dae8fc;strokeColor=#6c8ebf;" vertex="1" parent="1">
          <mxGeometry x="90" y="190" width="280" height="140" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-4" value="&lt;font color=&quot;#ff8000&quot;&gt;&lt;b&gt;QUESTION&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="190" y="160" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-5" value="&lt;font color=&quot;#009900&quot;&gt;&lt;b&gt;GOLD ANSWER&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="180" y="530" width="120" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-14" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-6" target="CBzDvX9ltago5Vxs7Bon-12">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-6" value="&lt;div&gt;&lt;font color=&quot;#009900&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;b&gt;Thought:&amp;nbsp;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;To find the dot product of two vectors, we need to multiply their corresponding components and then add them up.&amp;nbsp;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Do you know the Wolfram Alpha command to calculate the dot product of two given vectors?&lt;/font&gt;&lt;/div&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#fff2cc;strokeColor=#d6b656;" vertex="1" parent="1">
          <mxGeometry x="560" y="200" width="370" height="160" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-7" value="&lt;font color=&quot;#3333ff&quot;&gt;&lt;b&gt;QUERY GENERATOR&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="675.93" y="160" width="155" height="40" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-10" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;&amp;nbsp;The dot product of $\\begin{pmatrix} -2 \\\\ 0 \\\\ 7 \\end{pmatrix}$ and $\\begin{pmatrix} 3 \\\\ 4 \\\\ -5 \\end{pmatrix}$ is\n\\[(-2)(3) + (0)(4) + (7)(-5) = \\boxed{-41}.\\]&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#d5e8d4;strokeColor=#82b366;" vertex="1" parent="1">
          <mxGeometry x="80" y="360" width="300" height="160" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-11" value="&lt;font color=&quot;#7f00ff&quot;&gt;&lt;b&gt;FINAL QUERY TO API&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="760" y="620" width="107.03" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-3" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-12" target="CBzDvX9ltago5Vxs7Bon-14">
          <mxGeometry relative="1" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-12" value="&lt;div&gt;&lt;font color=&quot;#009900&quot; style=&quot;font-size: 16px;&quot;&gt;&lt;b&gt;Answer:&amp;nbsp;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;Yes, the Wolfram Alpha command to find the dot product of $\\begin{pmatrix} -2 \\\\ 0 \\\\ 7 \\end{pmatrix}$ and $\\begin{pmatrix} 3 \\\\ 4 \\\\ -5 \\end{pmatrix}$ is: &lt;b&gt;&lt;font color=&quot;#009900&quot;&gt;&lt;br&gt;&lt;/font&gt;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;b&gt;&lt;font color=&quot;#009900&quot;&gt;dot product [-2,0,7] and [3,4,-5]&lt;/font&gt;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;font style=&quot;font-size: 16px;&quot;&gt;&lt;br&gt;&lt;br&gt;&lt;b&gt;&lt;font color=&quot;#009900&quot;&gt;Final Query:&lt;/font&gt;&lt;/b&gt; dot product [-2,0,7] and [3,4,-5]&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#ffe6cc;strokeColor=#d79b00;" vertex="1" parent="1">
          <mxGeometry x="527.5" y="400" width="435" height="180" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-8" value="" style="edgeStyle=orthogonalEdgeStyle;rounded=0;orthogonalLoop=1;jettySize=auto;html=1;" edge="1" parent="1" source="CBzDvX9ltago5Vxs7Bon-14">
          <mxGeometry relative="1" as="geometry">
            <mxPoint x="500" y="735" as="targetPoint" />
          </mxGeometry>
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-14" value="&lt;font style=&quot;font-size: 16px;&quot;&gt;the dot product of [-2,0,7] and [3,4,-5] is -41.&lt;br&gt;&lt;/font&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f8cecc;strokeColor=#b85450;" vertex="1" parent="1">
          <mxGeometry x="625" y="690" width="240" height="90" as="geometry" />
        </mxCell>
        <mxCell id="CBzDvX9ltago5Vxs7Bon-15" value="&lt;div&gt;&lt;font color=&quot;#6666ff&quot;&gt;&lt;b&gt;WOLFRAM ALPHA API&lt;/b&gt;&lt;b&gt; +&amp;nbsp;&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;&lt;div&gt;&lt;font color=&quot;#6666ff&quot;&gt;&lt;b&gt;LLM ANSWER EXTRACTOR&lt;/b&gt;&lt;/font&gt;&lt;/div&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="680" y="790" width="170" height="70" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-5" value="-&lt;font style=&quot;font-size: 16px;&quot;&gt; We call the Wolfram Alpha API to find the dot product of the given vectors.&lt;br&gt;- The answer from Wolfram Alpha is -41.&lt;br&gt;- Therefore, the answer is $\\boxed{-41}$.&lt;/font&gt;&lt;br&gt;" style="rounded=1;whiteSpace=wrap;html=1;fillColor=#f5f5f5;strokeColor=#666666;fontColor=#333333;" vertex="1" parent="1">
          <mxGeometry x="130" y="655" width="370" height="160" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-6" value="&lt;font color=&quot;#a680b8&quot;&gt;&lt;b&gt;SOLUTION GENERATOR&lt;br&gt;&lt;/b&gt;&lt;/font&gt;" style="text;whiteSpace=wrap;html=1;" vertex="1" parent="1">
          <mxGeometry x="230" y="820" width="155" height="40" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-9" value="" style="shape=image;imageAspect=0;aspect=fixed;verticalLabelPosition=bottom;verticalAlign=top;image=data:image/png,iVBORw0KGgoAAAANSUhEUgAAARoAAACzCAMAAABhCSMaAAAAhFBMVEX///8AAAD09PT8/PwEBASEhITs7Ozl5eU6Ojrd3d2JiYkwMDDY2Nj5+fnw8PD39/evr6/CwsLMzMxbW1sWFhZKSkqgoKCQkJBmZmZzc3MqKio2Nja1tbWkpKRubm4fHx97e3vIyMhERERVVVVAQEASEhKYmJgcHBy0tLSPj49JSUklJSXEBIlEAAAKnklEQVR4nO2diZbaOgyGAw5L2HeYhW2AzLS8//tdbMmOEyLgnmKF9ui/tz3FJEz8IcuyvEwUicpVr/oBXleChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgIfWKaJQyf1f9GK+I5kX0Smi0nbTGy9Wxuz23p411r1rDeSU0UStt13zNdpMKn+aF0PSmhkd8+S9Td1TZ87wMmtamVqILpY9xRS75VdD8AIcyNrVVv5JHqgCNMYHmPn07tN+7x2ljlCi1syTiAhajba8Ku6nEagbrec40ukePw2naWSwW6ebDRzSu4CkrQNPa1UqlLWa7TNx1g89DZjoVsGFHM+yUg9EMvkd+u7n8u7dyb/e4H5QdzX5Lu9vGMH+t5jSe4bunAfOTsqK5dDS/yqGYvz9Lbxoc8LoptytmtRq18fug9m6ZpkvXZMpbzAXHCtlxB3+MaJTKwt3Tbo/BSoo2c2NIYOkxNyk+NCrauBa0qJuCy/+tuybRj/pduLHD9qxGjFazNG7l8mflff1gSLXNTUeSVGI2fGgm1qksvMI9ljVv3aki7PBHrJ6YDY3aIoW9X4oh79pdVX5z/WTsbf5volmim8mFtQso/PDGj6pM1mxaXE+rxYWmiQHM2v/ibWGGK523y3TEFFd56BNIXGgaNm7z9VYsLM3ZeJrr4IerUTGhMc6i2CKsY3YjyvEdMjqxNRpef3qgZ+b5MZ9Qs1+5wjkUNuDVxRi6d9AYff/wPDILGhfs5/voEZTNhvaqxSNkdLPi8cY8aPpQp1XuJ2Mbc3HwoJDkI5qUvoQle8PToDCc9ToY1x8fXZHJcK06pdq9zU+IxmhR8kOeLR40P1AhvyHY4N8NK3v61TudIVfJ+ndmO7/I654mHjSQpjln9VbZ4MkWzHVzutNSvKzfOngnzoMGApi5V2L7aeeYR5rM4e4nTT6s3QT3NzxopkUvrLCfXtqC4VlX94EE8NCEhReM8c0h6RPEicY2nktTwASWdS0KmlzjoQ+zeffV/Uv/SNVYTcsNnpQruBQNHnMfpSPV54vT1xwKrz3nM/1fyV90xh/PfciieNBAG3i3RlHHJuFcy950YAmtvF+pv1/FSQHEg2aU747q0CJ28EqpKJvEpfSWa2vYvx2DduA8aLAqzjkY3zNzP/uRwVPeRR9gyJBEAcWCJsHh0pstMJHvdx+/9HphvVHs/vJLch37HkrTkE/NgablqohTAipq6MjEGkLZ8oArMvnEcP9cg7KAYkBTP7vJ29RWb3DSZbo9KDChbs/TxniiBF9NznBzzuk2cqzDPHfAz9a6+NiV9/27FN1av9LT2HrwVKw3Rjn25QjQnv383h4+L+T6ifBW8+M3jsyZmkT43rxfKwyedLAce54p+oKbl941AygK2X0Ht5r6DPNPAAjzEgq+9raKht8lg6ehmbRy+QqbRG557gY+LqQfDm41uGxkuwOHYc0D29kaosFd8a5Pf0YOZ8vjbBB2EUR9IdM2odE0sYcZYw40i22g3+qZd5tXodtBl//kPsW3IwUNMugKgdBodDR36adXLiLuOgod18zW1/f1zAI2l/tK4WZv1NT9663mnHmJI6BwaV3tZQyZ7tVdCoMdV3OFo6ZsBHq68szPVmA0CbQn09lM0Epc68FOuTy5AJO+zmt/wrVuRd+wiOr5CoxmATUCH7GBxpV1ypAGn5bdqGeloCGiDgDZ9v69gvMJoMBoIIeF2QibwJrYPnhiUCXE+HmWq3vPdeDmchyRhhxfhkVzcSd+37yE+sxxn5y2ozim5pRgtN52r3GkdQCQYHDdkLsXwqLBTtfGrApHU65THlhDuJb6gGudN8mtOMFZrF3AZw+MJil4hE94XeiUS/Pf0GJi53iV9VsffTNyN2/u/95U1qRWMAvctpHrlOOyQSLmSGPPMvqYC0xdmiP+i7N8e6hCltn1nClorKv/pQpVVNqzxLXdd87VjrFJDSJcgR4yqmFC4zmTHdRu5b7vqS64Ck9g/NAfgeON3LXGkHbrIuAgYmlQXheLGfNsHaixo1m90DRM7netUxdxcdhlUxyB059MbtgPdzEg+XAoTNPpRNczBt2+ArZn9x7m9kDnwPsOw6LBhFMucikuFR7MbC4009ntWliB40U4/SwrFmeRYyAFjoYhdZAbCoyxU/bXSBQ68EXWpbfyfnyRpQzD+uAoOBoMYXPZ7Sk4jPNHFwSxXdeT72N/QQ7Lms3MklkFXyMbGM2nDWm9itj1WLdlk1RDk45wQaPda3Z/Jc4fKzCaIbSeds4tNEgemWZDe4cxvC97LwZGU4Z11aFTWStI0viBi+r/vgWlMMzCwNcGzLgL5LGVOH+m0Ggm1giyIhX1PxukOvOclQBbLw5acbWn8DMKOGraZHsLbrcFSHX27GXZPAsKssTXOdPnKziaPSaAFw9FIQp6pDf7KjrmnTJOe9ZmDMdMhJ+9RG/zYBq35aePlZ2GONUdCiiJOebqg/+EgQ3S0kfsZgUWBurbe70dGwjrn0CDmczCdlRCe31ptuQcu/m556BgDPb9D3TeWmbuVnuc2JwZQdfKzEnG1yNtP9UFtNoldz9bDGiUXfB5qeR7ejPHYoZTBy+XU8sNE7Qgi1U6QfNk8azl22WxXO2r8zlJWqXqzaDjRhJXi/Ujlxjl2A3PgkbpaZZ7W52sXKDbx8ncXEpjDG2TY0MUExrwr6iYln8YCya98hmrDVhf6P0JWmz7vIf3duOiMMWlsOnkDEQpXJPCMU7gPFNicrjJBOTPVpomWNz+nJ+3CynW82uSxgxNgZRLzNisjjcjrtxcDctTMx8Itb9tM9ts2SIubdz5d9vTWgJPJaB40agBmMyx3ixVFr+MceSV2we0KSsMJmY0MCN3f70vbKrLpcCUi45K1reFEPcJaz9Q5XvRbAqpDH88oDCm1tPA/6DVuIVmN2M25XY1eGfdtI7WIXGd1MJ+ZCHunJzdHIVjajCbGe+n3rmOTEeRsKNp1u43qUZmH6bttBZn2KQbly6kDST+M0DNBGScXzruS9l1bbWVHoUm4+WX170zHs5XwfGoX9jRUJuRO26PkJPbPMZ5SmoVJ8faCreTq7yWigZTOiJsB91QWFQV5w3Dij7tONLixIBan+hhRKfP5YGNKjmKOXXNZZv66YXm+t01IO8oG/jnlNVkoqrONk89H/J7MU6ag0EySec1cuT53WlFPIFepoqOfR/RDsXQWfeWB9zmWzvNO5MqDn6v6kT83vkGnK1JTahmMtlPetd7pZhU2S8LGJYvJdEmsxtEZr9qxarw9ygkq1LfcuA/xbxc1aG5WEWymxXBvIVevPi4Kv7tG/VxJxsGHHfjV/llIFoVP4u2kGFrsh+PJ61XwqL1Ss/zAq7X1yuheTEJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgIVX/D52cYht/VtiLAAAAAElFTkSuQmCC;clipPath=inset(22.07% 31.91% 22.07% 32.27% round 13%);" vertex="1" parent="1">
          <mxGeometry x="810" y="150" width="30.3" height="30" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-10" value="" style="shape=image;imageAspect=0;aspect=fixed;verticalLabelPosition=bottom;verticalAlign=top;image=data:image/png,iVBORw0KGgoAAAANSUhEUgAAARoAAACzCAMAAABhCSMaAAAAhFBMVEX///8AAAD09PT8/PwEBASEhITs7Ozl5eU6Ojrd3d2JiYkwMDDY2Nj5+fnw8PD39/evr6/CwsLMzMxbW1sWFhZKSkqgoKCQkJBmZmZzc3MqKio2Nja1tbWkpKRubm4fHx97e3vIyMhERERVVVVAQEASEhKYmJgcHBy0tLSPj49JSUklJSXEBIlEAAAKnklEQVR4nO2diZbaOgyGAw5L2HeYhW2AzLS8//tdbMmOEyLgnmKF9ui/tz3FJEz8IcuyvEwUicpVr/oBXleChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgIfWKaJQyf1f9GK+I5kX0Smi0nbTGy9Wxuz23p411r1rDeSU0UStt13zNdpMKn+aF0PSmhkd8+S9Td1TZ87wMmtamVqILpY9xRS75VdD8AIcyNrVVv5JHqgCNMYHmPn07tN+7x2ljlCi1syTiAhajba8Ku6nEagbrec40ukePw2naWSwW6ebDRzSu4CkrQNPa1UqlLWa7TNx1g89DZjoVsGFHM+yUg9EMvkd+u7n8u7dyb/e4H5QdzX5Lu9vGMH+t5jSe4bunAfOTsqK5dDS/yqGYvz9Lbxoc8LoptytmtRq18fug9m6ZpkvXZMpbzAXHCtlxB3+MaJTKwt3Tbo/BSoo2c2NIYOkxNyk+NCrauBa0qJuCy/+tuybRj/pduLHD9qxGjFazNG7l8mflff1gSLXNTUeSVGI2fGgm1qksvMI9ljVv3aki7PBHrJ6YDY3aIoW9X4oh79pdVX5z/WTsbf5volmim8mFtQso/PDGj6pM1mxaXE+rxYWmiQHM2v/ibWGGK523y3TEFFd56BNIXGgaNm7z9VYsLM3ZeJrr4IerUTGhMc6i2CKsY3YjyvEdMjqxNRpef3qgZ+b5MZ9Qs1+5wjkUNuDVxRi6d9AYff/wPDILGhfs5/voEZTNhvaqxSNkdLPi8cY8aPpQp1XuJ2Mbc3HwoJDkI5qUvoQle8PToDCc9ToY1x8fXZHJcK06pdq9zU+IxmhR8kOeLR40P1AhvyHY4N8NK3v61TudIVfJ+ndmO7/I654mHjSQpjln9VbZ4MkWzHVzutNSvKzfOngnzoMGApi5V2L7aeeYR5rM4e4nTT6s3QT3NzxopkUvrLCfXtqC4VlX94EE8NCEhReM8c0h6RPEicY2nktTwASWdS0KmlzjoQ+zeffV/Uv/SNVYTcsNnpQruBQNHnMfpSPV54vT1xwKrz3nM/1fyV90xh/PfciieNBAG3i3RlHHJuFcy950YAmtvF+pv1/FSQHEg2aU747q0CJ28EqpKJvEpfSWa2vYvx2DduA8aLAqzjkY3zNzP/uRwVPeRR9gyJBEAcWCJsHh0pstMJHvdx+/9HphvVHs/vJLch37HkrTkE/NgablqohTAipq6MjEGkLZ8oArMvnEcP9cg7KAYkBTP7vJ29RWb3DSZbo9KDChbs/TxniiBF9NznBzzuk2cqzDPHfAz9a6+NiV9/27FN1av9LT2HrwVKw3Rjn25QjQnv383h4+L+T6ifBW8+M3jsyZmkT43rxfKwyedLAce54p+oKbl941AygK2X0Ht5r6DPNPAAjzEgq+9raKht8lg6ehmbRy+QqbRG557gY+LqQfDm41uGxkuwOHYc0D29kaosFd8a5Pf0YOZ8vjbBB2EUR9IdM2odE0sYcZYw40i22g3+qZd5tXodtBl//kPsW3IwUNMugKgdBodDR36adXLiLuOgod18zW1/f1zAI2l/tK4WZv1NT9663mnHmJI6BwaV3tZQyZ7tVdCoMdV3OFo6ZsBHq68szPVmA0CbQn09lM0Epc68FOuTy5AJO+zmt/wrVuRd+wiOr5CoxmATUCH7GBxpV1ypAGn5bdqGeloCGiDgDZ9v69gvMJoMBoIIeF2QibwJrYPnhiUCXE+HmWq3vPdeDmchyRhhxfhkVzcSd+37yE+sxxn5y2ozim5pRgtN52r3GkdQCQYHDdkLsXwqLBTtfGrApHU65THlhDuJb6gGudN8mtOMFZrF3AZw+MJil4hE94XeiUS/Pf0GJi53iV9VsffTNyN2/u/95U1qRWMAvctpHrlOOyQSLmSGPPMvqYC0xdmiP+i7N8e6hCltn1nClorKv/pQpVVNqzxLXdd87VjrFJDSJcgR4yqmFC4zmTHdRu5b7vqS64Ck9g/NAfgeON3LXGkHbrIuAgYmlQXheLGfNsHaixo1m90DRM7netUxdxcdhlUxyB059MbtgPdzEg+XAoTNPpRNczBt2+ArZn9x7m9kDnwPsOw6LBhFMucikuFR7MbC4009ntWliB40U4/SwrFmeRYyAFjoYhdZAbCoyxU/bXSBQ68EXWpbfyfnyRpQzD+uAoOBoMYXPZ7Sk4jPNHFwSxXdeT72N/QQ7Lms3MklkFXyMbGM2nDWm9itj1WLdlk1RDk45wQaPda3Z/Jc4fKzCaIbSeds4tNEgemWZDe4cxvC97LwZGU4Z11aFTWStI0viBi+r/vgWlMMzCwNcGzLgL5LGVOH+m0Ggm1giyIhX1PxukOvOclQBbLw5acbWn8DMKOGraZHsLbrcFSHX27GXZPAsKssTXOdPnKziaPSaAFw9FIQp6pDf7KjrmnTJOe9ZmDMdMhJ+9RG/zYBq35aePlZ2GONUdCiiJOebqg/+EgQ3S0kfsZgUWBurbe70dGwjrn0CDmczCdlRCe31ptuQcu/m556BgDPb9D3TeWmbuVnuc2JwZQdfKzEnG1yNtP9UFtNoldz9bDGiUXfB5qeR7ejPHYoZTBy+XU8sNE7Qgi1U6QfNk8azl22WxXO2r8zlJWqXqzaDjRhJXi/Ujlxjl2A3PgkbpaZZ7W52sXKDbx8ncXEpjDG2TY0MUExrwr6iYln8YCya98hmrDVhf6P0JWmz7vIf3duOiMMWlsOnkDEQpXJPCMU7gPFNicrjJBOTPVpomWNz+nJ+3CynW82uSxgxNgZRLzNisjjcjrtxcDctTMx8Itb9tM9ts2SIubdz5d9vTWgJPJaB40agBmMyx3ixVFr+MceSV2we0KSsMJmY0MCN3f70vbKrLpcCUi45K1reFEPcJaz9Q5XvRbAqpDH88oDCm1tPA/6DVuIVmN2M25XY1eGfdtI7WIXGd1MJ+ZCHunJzdHIVjajCbGe+n3rmOTEeRsKNp1u43qUZmH6bttBZn2KQbly6kDST+M0DNBGScXzruS9l1bbWVHoUm4+WX170zHs5XwfGoX9jRUJuRO26PkJPbPMZ5SmoVJ8faCreTq7yWigZTOiJsB91QWFQV5w3Dij7tONLixIBan+hhRKfP5YGNKjmKOXXNZZv66YXm+t01IO8oG/jnlNVkoqrONk89H/J7MU6ag0EySec1cuT53WlFPIFepoqOfR/RDsXQWfeWB9zmWzvNO5MqDn6v6kT83vkGnK1JTahmMtlPetd7pZhU2S8LGJYvJdEmsxtEZr9qxarw9ygkq1LfcuA/xbxc1aG5WEWymxXBvIVevPi4Kv7tG/VxJxsGHHfjV/llIFoVP4u2kGFrsh+PJ61XwqL1Ss/zAq7X1yuheTEJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgISVoSAkaUoKGlKAhJWhICRpSgoaUoCElaEgJGlKChpSgIVX/D52cYht/VtiLAAAAAElFTkSuQmCC;clipPath=inset(22.07% 31.91% 22.07% 32.27% round 13%);" vertex="1" parent="1">
          <mxGeometry x="980" y="390" width="30.3" height="30" as="geometry" />
        </mxCell>
        <mxCell id="ufljFMe3RaCTCH4WWNqV-16" value="" style="shape=image;verticalLabelPosition=bottom;labelBackgroundColor=default;verticalAlign=top;aspect=fixed;imageAspect=0;image=data:image/png,iVBORw0KGgoAAAANSUhEUgAAAGIAAABkCAYAAAB9/OUTAAAMamlDQ1BJQ0MgUHJvZmlsZQAASImVVwdYU8kWnltSSWgBBKSE3gSRGkBKCC2A9CLYCEkgocSYEFTsZVHBtYsI2NBVEcW2AmLHriyKvS8WVJR1URcbKm9CArruK987+ebeP2fO/KfcueUAoPWBJ5XmodoA5EsKZAnhwczRaelM0jOAwJ8+IAN7Hl8uZcfFRQMoA+e/y7sb0BbKVWcl1z/n/6voCoRyPgDIWIgzBXJ+PsTHAcCr+FJZAQBEpd5qcoFUiWdDrCeDAUK8SomzVXi7Emeq8OF+m6QEDsSXASDTeDxZNgCa96CeWcjPhjyanyF2lQjEEgC0hkEcwBfxBBArYx+Wnz9Ricshtof2UohhPICV+R1n9t/4Mwf5ebzsQazKq1/IIWK5NI839f8szf+W/DzFgA9bOGgiWUSCMn9Yw1u5E6OUmAZxlyQzJlZZa4g/iAWqugOAUkWKiGSVPWrCl3Ng/YABxK4CXkgUxCYQh0nyYqLV+swscRgXYrhb0CniAm4SxIYQLxTKQxPVNhtlExPUvtD6LBmHrdaf48n6/Sp9PVDkJrPV/G9EQq6aH9MsEiWlQkyF2LpQnBIDsSbELvLcxCi1zcgiESdmwEamSFDGbw1xglASHqzixwqzZGEJavuSfPlAvthGkZgbo8b7CkRJEar6YKf4vP74YS7YZaGEnTzAI5SPjh7IRSAMCVXljj0XSpIT1TwfpAXBCaq1OFWaF6e2xy2FeeFKvSXEHvLCRPVaPKUAbk4VP54lLYhLUsWJF+XwIuNU8eDLQDTggBDABAo4MsFEkAPErV0NXfCfaiYM8IAMZAMhcFZrBlak9s9I4DERFIE/IBIC+eC64P5ZISiE+i+DWtXRGWT1zxb2r8gFTyHOB1EgD/5X9K+SDHpLAU+gRvwP7zw4+DDePDiU8/9eP6D9pmFDTbRaoxjwyNQasCSGEkOIEcQwogNujAfgfng0PAbB4YazcJ+BPL7ZE54S2giPCNcJ7YTbE8RzZT9EOQq0Q/4wdS0yv68Fbgs5PfFg3B+yQ2bcADcGzrgH9MPGA6FnT6jlqONWVoX5A/ffMvjuaqjtKK4UlDKEEkSx/3GlpqOm5yCLstbf10cVa+ZgvTmDMz/653xXfQE8R/1oiS3E9mNnsRPYeeww1gCY2DGsEWvBjijx4O560r+7Brwl9MeTC3nE//A3cGWVlZS71rp2un5WzRUIpxQobzzOROlUmThbVMBkw7eDkMmV8F2GMd1c3dwBUL5rVI+vt/H97xDEoOWbbt7vAPgf6+vrO/RNF3kMgL3e8PY/+E1nzwJARwOAcwf5ClmhSocrDwT4lNCCd5oRMANWwB7m4wa8gB8IAqEgEsSCJJAGxsPoRXCfy8BkMB3MAcWgFCwDq0EF2AA2g+1gF9gHGsBhcAKcARfBZXAd3IW7pwO8BN3gHehFEISE0BEGYoSYIzaIE+KGsJAAJBSJRhKQNCQDyUYkiAKZjsxDSpEVSAWyCalB9iIHkRPIeaQNuY08RDqRN8gnFENpqB5qitqiw1EWykaj0CR0HJqNTkKL0PnoErQcrUZ3ovXoCfQieh1tR1+iPRjANDADzAJzxlgYB4vF0rEsTIbNxEqwMqwaq8Oa4HW+irVjXdhHnIgzcCbuDHdwBJ6M8/FJ+Ex8MV6Bb8fr8VP4Vfwh3o1/JdAJJgQngi+BSxhNyCZMJhQTyghbCQcIp+G91EF4RyQSDYh2RG94L6YRc4jTiIuJ64i7iceJbcTHxB4SiWREciL5k2JJPFIBqZi0lrSTdIx0hdRB+kDWIJuT3chh5HSyhDyXXEbeQT5KvkJ+Ru6laFNsKL6UWIqAMpWylLKF0kS5ROmg9FJ1qHZUf2oSNYc6h1pOraOept6jvtXQ0LDU8NGI1xBrzNYo19ijcU7jocZHmi7NkcahjaUpaEto22jHabdpb+l0ui09iJ5OL6AvodfQT9If0D9oMjRdNLmaAs1ZmpWa9ZpXNF9pUbRstNha47WKtMq09mtd0urSpmjbanO0edoztSu1D2rf1O7RYeiM0InVyddZrLND57zOc12Srq1uqK5Ad77uZt2Tuo8ZGMOKwWHwGfMYWxinGR16RD07Pa5ejl6p3i69Vr1ufV19D/0U/Sn6lfpH9NsNMANbA65BnsFSg30GNww+DTEdwh4iHLJoSN2QK0PeGw41DDIUGpYY7ja8bvjJiGkUapRrtNyowei+MW7saBxvPNl4vfFp466hekP9hvKHlgzdN/SOCWriaJJgMs1ks0mLSY+pmWm4qdR0relJ0y4zA7MgsxyzVWZHzTrNGeYB5mLzVebHzF8w9ZlsZh6znHmK2W1hYhFhobDYZNFq0WtpZ5lsOddyt+V9K6oVyyrLapVVs1W3tbn1KOvp1rXWd2woNiwbkc0am7M2723tbFNtF9g22D63M7Tj2hXZ1drds6fbB9pPsq+2v+ZAdGA55Dqsc7jsiDp6OoocKx0vOaFOXk5ip3VObcMIw3yGSYZVD7vpTHNmOxc61zo/dDFwiXaZ69Lg8mq49fD04cuHnx3+1dXTNc91i+vdEbojIkfMHdE04o2boxvfrdLtmjvdPcx9lnuj+2sPJw+hx3qPW54Mz1GeCzybPb94eXvJvOq8Or2tvTO8q7xvsvRYcazFrHM+BJ9gn1k+h30++nr5Fvju8/3Tz9kv12+H3/ORdiOFI7eMfOxv6c/z3+TfHsAMyAjYGNAeaBHIC6wOfBRkFSQI2hr0jO3AzmHvZL8Kdg2WBR8Ifs/x5czgHA/BQsJDSkJaQ3VDk0MrQh+EWYZlh9WGdYd7hk8LPx5BiIiKWB5xk2vK5XNruN2R3pEzIk9F0aISoyqiHkU7Rsuim0ahoyJHrRx1L8YmRhLTEAtiubErY+/H2cVNijsUT4yPi6+Mf5owImF6wtlERuKExB2J75KCk5Ym3U22T1YkN6dopYxNqUl5nxqSuiK1ffTw0TNGX0wzThOnNaaT0lPSt6b3jAkds3pMx1jPscVjb4yzGzdl3PnxxuPzxh+ZoDWBN2F/BiEjNWNHxmdeLK+a15PJzazK7OZz+Gv4LwVBglWCTqG/cIXwWZZ/1oqs59n+2SuzO0WBojJRl5gjrhC/zonI2ZDzPjc2d1tuX15q3u58cn5G/kGJriRXcmqi2cQpE9ukTtJiafsk30mrJ3XLomRb5Yh8nLyxQA9+1Lco7BU/KR4WBhRWFn6YnDJ5/xSdKZIpLVMdpy6a+qworOiXafg0/rTm6RbT50x/OIM9Y9NMZGbmzOZZVrPmz+qYHT57+xzqnNw5v811nbti7l/zUuc1zTedP3v+45/Cf6ot1iyWFd9c4Ldgw0J8oXhh6yL3RWsXfS0RlFwodS0tK/28mL/4ws8jfi7/uW9J1pLWpV5L1y8jLpMsu7E8cPn2FTorilY8XjlqZf0q5qqSVX+tnrD6fJlH2YY11DWKNe3l0eWNa63XLlv7uUJUcb0yuHJ3lUnVoqr36wTrrqwPWl+3wXRD6YZPG8Ubb20K31RfbVtdtpm4uXDz0y0pW87+wvqlZqvx1tKtX7ZJtrVvT9h+qsa7pmaHyY6ltWitorZz59idl3eF7Gqsc67btNtgd+kesEex58XejL039kXta97P2l/3q82vVQcYB0rqkfqp9d0Noob2xrTGtoORB5ub/JoOHHI5tO2wxeHKI/pHlh6lHp1/tO9Y0bGe49LjXSeyTzxuntB89+Tok9dOxZ9qPR11+tyZsDMnz7LPHjvnf+7wed/zBy+wLjRc9LpY3+LZcuA3z98OtHq11l/yvtR42edyU9vItqNXAq+cuBpy9cw17rWL12Out91IvnHr5tib7bcEt57fzrv9+k7hnd67s+8R7pXc175f9sDkQfXvDr/vbvdqP/Iw5GHLo8RHdx/zH798In/yuWP+U/rTsmfmz2qeuz0/3BnWefnFmBcdL6Uve7uK/9D5o+qV/atf/wz6s6V7dHfHa9nrvjeL3xq93faXx1/NPXE9D97lv+t9X/LB6MP2j6yPZz+lfnrWO/kz6XP5F4cvTV+jvt7ry+/rk/JkvP5PAQwONCsLgDfbAKCnAcCAfRt1jKoX7BdE1b/2I/CfsKpf7BcvAOrg93t8F/y6uQnAni2w/YL8WrBXjaMDkOQDUHf3waEWeZa7m4qLBvsUwoO+vrewZyOtBODLsr6+3uq+vi+bYbCwdzwuUfWgSiHCnmFj6JfM/Ezwb0TVn36X449noIzAA/x4/heI9JDOiDAm9QAAAIplWElmTU0AKgAAAAgABAEaAAUAAAABAAAAPgEbAAUAAAABAAAARgEoAAMAAAABAAIAAIdpAAQAAAABAAAATgAAAAAAAACQAAAAAQAAAJAAAAABAAOShgAHAAAAEgAAAHigAgAEAAAAAQAAAGKgAwAEAAAAAQAAAGQAAAAAQVNDSUkAAABTY3JlZW5zaG905TzaowAAAAlwSFlzAAAWJQAAFiUBSVIk8AAAAdVpVFh0WE1MOmNvbS5hZG9iZS54bXAAAAAAADx4OnhtcG1ldGEgeG1sbnM6eD0iYWRvYmU6bnM6bWV0YS8iIHg6eG1wdGs9IlhNUCBDb3JlIDYuMC4wIj4KICAgPHJkZjpSREYgeG1sbnM6cmRmPSJodHRwOi8vd3d3LnczLm9yZy8xOTk5LzAyLzIyLXJkZi1zeW50YXgtbnMjIj4KICAgICAgPHJkZjpEZXNjcmlwdGlvbiByZGY6YWJvdXQ9IiIKICAgICAgICAgICAgeG1sbnM6ZXhpZj0iaHR0cDovL25zLmFkb2JlLmNvbS9leGlmLzEuMC8iPgogICAgICAgICA8ZXhpZjpQaXhlbFlEaW1lbnNpb24+MTAwPC9leGlmOlBpeGVsWURpbWVuc2lvbj4KICAgICAgICAgPGV4aWY6UGl4ZWxYRGltZW5zaW9uPjk4PC9leGlmOlBpeGVsWERpbWVuc2lvbj4KICAgICAgICAgPGV4aWY6VXNlckNvbW1lbnQ+U2NyZWVuc2hvdDwvZXhpZjpVc2VyQ29tbWVudD4KICAgICAgPC9yZGY6RGVzY3JpcHRpb24+CiAgIDwvcmRmOlJERj4KPC94OnhtcG1ldGE+Cqg7v7wAAAAcaURPVAAAAAIAAAAAAAAAMgAAACgAAAAyAAAAMgAACjI/3TbtAAAJ/klEQVR4Aexba5AUVxX+ume65/3a2Z1d9hGWZzZZhY0RDIoxxoI8REoEI5AfMQkFRKPEVBSrfJZIjMZHEstYEMrCWBhKJQQtK2JVSqiowSImUuCCkIdAgCz7mGF3dmdmZ7rb07PMbPd090z37Iw7W7X3T9977jn3nj5f33vuPfc2I1HCdJp0CzDTQEw6BlkFpoGoDRwwDcQ0EDVigRpRY3pETANRIxaoETWmR8Q0EBWygJBB9NmfInTvlyrU4OQ0M+VHxJXf7AIGesHO74Tv1pWTY8UK9DqlgUhfPIfh/b8EY7NDzKQR+OxDYL3+Cpjl/9/ElAYiuvP7YEUxbzXJF0Tw7gfy5amUmbJAjPzzr0gffVlja/edd4G7Zo6GXuuEqQmEJCL29KM0Jdk09hWpLvTA1zT0WidMSSBi+34BprfH0Lbste+F76MrDOtrsWLKAZHp70F8786sgzYy6FR03FUFomfXU/B0dsK75GNGNrNMj+56HGwmU1JO8ocQXL+5JJ9ZhoHf74UNIgIr15sVscRXVSBOf3ETHEMX4WoMg1v4AQQ/vQGMnbOkoJLZyEEreZT5iTruDO1P+n/3LIaPHAZrY+BftAR1G7+q7KJi+aoCceaRLRj828toe/9csLz8PTFgZ85DYO0mcJFmay9BTjj69HfJIOaBLNdxJ06fQN+enUi//SbpKGUXBd6gB8477oJv+aes6W2Su6pAXNj5M1zc9Qx4rwstN7SrVJKC9fDcthruxbeo6EaFUg7aSI7tWADfLR83qh6n04lx9E/PY/DgCxAG+sfpDANXwAOOs8G16j54li4br6tgrqpAXH7htzj76Pasup7GICLzZ2hUFzkHuK4lCK65n6Ytu6ZeJow56B30ZZofDbmGso773ofBerw5kuqZifZhYN+vMPLKIYjptKpOLvA+F5xOPkv3f+E74NvnaXgqQagqEMMnjqH7vnvyetZf2wJfRD8EkZ222ufTtLUZXENTXkbOmHXQKiFFQQrUIbhuk4ICJM50o3/PDoy+dUZFVxZYBwev350n1f/ouXy+0pmqAgEKPxy96X15nVkbi+auWeDcY19YvqIwE2qA+7Y1cC+6GVYddGFTubJrxTrwre2IHqTp58X96uknx6R4yptFX516FE1dIOjFji7uUrweYHc60LZotopmVJCnLVtjK+wujxGLaXqirw/Jt9/QnX40jZBf8IS8sNGHk0uyLpHHdueKFX9Wd0SQuv9a/hGkY1dUihv5CxVTrkDLXW7mfNByKUex/ByN9iN+6iTMXuFy+NxwONX+SHJ70bDtGct9mxWoPhC334r0wIBGn2L+opBZohHBt5YXyJNGU4gde93cSKCObeSYPeSgNYlGZv1XHteQK0WoOhDd61dj+A15Pa5Osr+YQf6CL+UvcmIB2hRGWnIl08/Y669CSCRM8ev5hZwgM6sD4Qe/lStW/Fl1IM5s2YzYK0d0FZf9RcvCmdnNni5DITHSCo5WQGbT0H+6Mdqv2BMUEyS/4KvzgWEZXS77gsUI3lO949jqA/HlhxA7fEj35WSiK+xD0/WthvWqCsYGW9tssA6dqUPFSMvTd85h5NzZAqpx0UmbNp7X38fIUo7bPwPfsk8aNzDBmqoD8e5zu3H+J08UVbP5uibwAfoaOWND5Bsw4bwtOWcKncjTpDccyHehl3Gv2QB3BYOXhX1UHYjLB/bh7PZthf2qyo1tXrhtAiQysuj1wUYrFCiWjipmKhRz3qacMxk/MzqKTDwOaTQNZ0MdAjMihd2oyoGtPyYfpY0MqJgmUKg6EMlz/8XxNcWHdKTNB49NHdoWHU7A7QbrMgDFwHkbOmeKJQkUwkgPDWaNr7SZGSCquZmTdak6EIW7a6UBcnk9IHJ18jMLisdH8aKCjV2B89Y456vGF5IJCMMjyiZV+VJASOTIG374a5VMpQvVB4I0fpXCHJLitkXhS5QCIs/PsBBcTjBOzxgoCuetdM5imqYdWrIWM36+TcqUAkLkaVf9vd1KkYrnqwKEGL9C0cyXkDryF4hn/o2+y0nEB4y/SNNAKF//KigIhsHUt2Kw+zgZPwlhhPopArqyiVze29IETziYK2qeEo1Ge8sc2Ooj4OZ2wrVwsYZnooSJA0HDf/jQH5F67e8Q3joJ0KUvJjWq0kuUGFyI88ik1H4gx1QWEDlheiYYDoMDQwqKtWxgVhucvoJp72oTEsuCb5uraVCUf3iTFxZ0wOXo6IJj3vUaHisEy0CkTh9H4vCLSJ86BunSObCxmKn+kuBwqW/8MphSqGaBIGPbm2eB4dVxJ6XuyrxIoMEXgn3mHDiv6wLXaD4SUBSITO+7iL90AJmTr0F68xRARmcsDnulolHRjdhASknK5msWCLqAwFFIvtwk0TJZtDvA1jWAm90BV2cXXQnV368UBSK24zFkDuwpVw9duUtJN5JxNRi1CITE8eCb23XfoRyiKAhw3HwH3Dd+SFe8KBCyRP+T34R0cL+ucDlE2V+cj9FFAkGeZMdSoN6NOu94OUc3+6y0j5BPC/kZ7aanJDN6suRHfMtXGbKWBEKW7H14HZhTJwwbsVoxAh49fUJezBt0oiGoH2zLMxXJVBQI+h7Y+ibYKnirnJk1H/5P3F3kDSxs6C5vXAH2HfNBtKK9UmVvxo14bGyKqiUgsuGTMsLtRu8rhpsQMnFD3dSIyHZCjqdnw52wXbpg1Kdl+vkhR3ZJWytAiHQK6Ggr7wBK7+VFhxuhTVv1qjQ080CQqEQ/g/SuXQpW3jRVIKXpEuPFKAO3zzGpU1NoTjsdUDktLVVLvX6Gfp4Jf+7rNOeYm3ItASF3Li9pBzavBGvy1KuUwlckF0YFdlKBaFzQATYYgS1gvLsu9R7Ketn71X3+GxRBNhHWvypoGQhZTv5lKvrgarDJ5NVmJva4wvkRcOhv9sy0PFFnHVl0A/imNjNdleQRRQGB+x8BS38vWUllASF3MPKPQxjZtsVyXEepHN0qRZKGLtM0A45QGNJgjHbq2osGShm9fDlAMHTe4QqH4Aj6Yac7TKybrlU2z9Rr3jRNoFvqfvqPz04bOKupbCDkjuIU6kj8YKscS7fUb5KipqOktDCShL0hDH/ngnF5CuKIqYQlUMwCwdrp/mokDN7vBc8pwxYSJDrbZihqmz2YammHPVQ/rpOJnBxd9qzdCK7MkTUhIGT9hv78PJJPfrskGGmKliYFOhlLpMjpj+0hWLq6Erzpg3RgTzEavWQSlGJAGBtf3aF8c5ztuUwjfEw3ul0GkUYp13INhdz1r4nmWpB3zc5lq+B6z405kuXnhIGQe4z+fDuEP+zVdC7QtJOinXRKNj4dSRam0NIP0w0O5ZdZyKEoFwGlEAizxle0ns0K9PO8rUf7S5gk60hRVjmIx8gnh4pUKnShYC2a/R8AAAD//5pJqsIAAAtaSURBVO1beXRU1Rn/zfJmSWbLTHYSllA4LSCbLAFUAihUESuiolalRWh7wKpHmrbU4x9Ki7v2WCxHqLan0nJs6SkeipadhoI5slilkCISIgnJJMxkklmYyaz93pCZzPLevDcbND3cf+be737Lffd33/fd7943khAV5KBYX/0pQvt3IgQJPBIJvF4/Apc9vJq1N06GQm/g7RfqCPSRbqcd0u5uuEMSql6GutQEhU4DBcMIifP2B0mv1Grl7y8ohLS0HEzlsDCPdPw0aOsW8vKL7ZDkCgjW4PkltfB3WRAKpsZWNWIYCkeMFDtGQT6fzwe5lx90QQUJDKFeGySuywnUhKZUglDlUJS8uiWhI7NmzoBoWXEHvE1nBEchL9JBP2mKIJ9YhqCMgaK8Gt7zTZD4vGLFBPhoIVkuAV6fAB8gXXA3jN9dI8gnxJATIFrXroC74YCQLUgZOfQzZ0EqkwnyimFgXzxFVc0VVm8f+lr+A6kYQRE8wVAQ0s4uIBgQ5GYWLoX+kccF+VIxZA2E+c3nYH//96lsRPv0s2ZCrlRF21lVKLTJy6oBRhFVE7B3I2i+QG1JlJZNJej3Q9rVKUoFc88y6O9fIYqXiykrIMwb18O+5R0uvUk0zcQJUBpNSfRMCRKtATKdMUncS0BI7LYkeqaEoMsJaW+vsDhhr35qHQqn1wnzcnBkDETvwZ3ofOYJDpXJJGV1JTSjvp7ckSElEhf4xHMbL4CQ1QJJXx+fuQE6BXBN/ctQTaodoImsZQSE/dBumH+2ivxn6t0ROwY2OOsmTIZEmhvvHRcX+B4yx/GCoADM5KJExAsQGLp1m6AYmd7CSxsIZ+NBtNeTLxQBAhucdbW1kMX4cb65E0XniAt8crmOF4FgEDJzB5+5OHqI4mDRa1sgLy6Lo6dqpAWEt6MVLQ/eCvj8qXSG+zxKNYLGcpQMr4BKpaT4mX0A5YsLfIPJXbwIoa/PB3ubGQWMFIVy4WcJqdUwvrEVMoO4uCgaCF9XB1oevhUhF3/idFmhRk9AgW6njzLrgT04Q2/G0JpKmMqKoDVQZprB9lUoLvCCkWF+wb4BbrsL3RfNsF7sQpDakaJQKqAjl2syaKBR8LvckLoAJe98RMkGP09Epygg/DYLzi+tIxDcEbnwb4h8Jzv5Nr8CNoePXhThN4UVNBRpUVVTAYNJB3WhOk4nV0NUXOASZGmi40UIHrcXvXQyYGs1w+UUyKz77TF0nBIGpUgDrTI5PwpWDEHp61sFPYIwELQSmh+aDX9re9g0ezTlZApgC8jRQ5PvDwgnPP1j5vyRSqQYRqAUVxihpYeRyeXxfGnEhXjBgRZfvPDTwnH3OmEll2PtoEw6y8KOXU+LzEhvil5F5139Hiw4ZChKX/tDSu2CQDQ/VAdfSyscjAo2H4Mepxfsa5uvotUUoGpkJYpK9SikerpxgW9c/q52BG1d8JBr7em8BFtbJ9xufjfLp0csXUbuV2vQwkSLS69mIBk3GcXPvskrnhKI5nX1OPvh7vDk5+iQlncgsR1GfSE0FFcYpRIjF86BTJF9Nu6nxMyyYxt8UgZ2hweOBDcbaz/XdSnFCK1eg6/VP4viux/iVJ8SCFbCb+9F+95dsDQega2pCU6zmVaSiOSG0xw3US6XwagtgFomRZB2J4H+XRlToESfVodJi2inlkUJBfz4YtvfYfCaB7SQTZ9Ujl6XFw5nfOwbYMq8xrqpwrJyaMfeAOPN81A2fyFk9Cx8RRAILkHXuTPo2LcH3SeOw/blOTitNrBH0ekUlYKBQauGihypn4CN3ZVE9LBAnLf04sbbZqH8G6Mj5LR/uz49iY7j/0a50sUtS0mYX87A4fahx54+KBJ6BhXdg2iG10A/pRYlt90ZTmK5jXFTMwIiUVXI44b1WCMshxvQffJz9H7VBicFwUBsJkpBV0c+X6dWgqEg1ucQ3pUoClRotvSQuRDmP3Y/mEJNomnBtsdiwZnte8J8vEAkaAnQTsjVFwiDEqBxJ5b41T6HVvuilKs9UZ6rnRMguBR7zW3ooqNx67GjcH32KV20uOHzpH9f0NZ/y2cqL8b0JbdDIkvYVXEZ76exLun0Hz+Av++KXbFAxKoMkotxBWjl0HG7ftoMlMy9HfqJubtPidjKGxARA+xvw5Txsc206hEgWKGxMydh+JSJouXbDh6B9cuvwvwSyuzLFE7RsrGMEtr9jNr5r1hSzuv5B4K2ug3TxE9e4hPGAsH2zXvkbqiKihLZktqOlgto3ns4SpdKZShl7NF2WhWKIaMPfZmWSLrMeQfCeepznFj2cLrjivInAqFSqzB3+X0pXVSQ7q9Pb/0b7b4GNhAy2iWVyDIEgkYz+vC56JjyUck7EOYPtuGLdc9nPPZEIFhFI8aNwpi5N/HqbN6xFw5K2mILQ4d1JqkjlpRWffif9kMxZFhaMukw5x2IC5veQsumt9MZUxwvFxAsw8zF81FUPSSOl210N51F6+FjSXQVE4RBmv7WNKKoeO16GO9cGmnm/DfvQDTVP4VLB/ZnPPB2D5tjJG8hGYUC85Yvicu62ez51NYdnLbUyhD0EN4ycwoT0fjkWhRncSfNpzdCzzsQp5/4PixHPo7YS/vXTFtPf4D7bKu0sgxT770jrDOSPXsc3O6HckPowJPQiRiV+pY5qH7hNyI4M2PJOxDHFy+Eq7U1s9GRVCcFXJ+P/4R38q2zUDFmNCLZM5+hAjVdYQYz276yOlXTZ2Do61v41GdNzzsQnyyog8fanfFArXTM7qbzp1RlGoHRfuR4KhYUFtLBm5/7bUkp2N8prxmOmvf2iWHNiCfvQDTOroVX6PPFFEPvpWMShyc1EGV0B8AIgJUtEBKjHqN2nEgx0uy68g5Eplk1+9WHYcIEnPvsJC47U7sUMUBoq+hGUBeE71xzRjOW7+w6r0CE6FvUQzPSO5eR0R1ExV3fQtWKH0BhKoa96RQ+vO8ezp1TZEaFgGDvyKfTvQpjKoHvUgfMr6yF59jHCPX5IypE/eYzqcsrEDY6jT35pLhvQgsqK1G17DsoX/JA0qQ0rv4emg8cTKJHCEJAVD3wIGp+tDbCfuWXvm01b/g5HLv+ipBNXMY9+tBZUR8CxBsS18orEB1/eR9nX/gF70jYlaobdwNqnq6Hhi5Q+Irf5cKOuplw89yqpQJCbTJh6q4DfKrDdPaDOcuml+BvbknJV7X5zygYMzklT6adeQXiwsZfoeWdzUljk5P7KVu0CNUrV4XdTxIDB6F5y+/QuH49Rw+QCogJGzdBP7WWUy6R6Otsh/nVtXDT3QrojzaJxfST52G669uJ5Jy08wpE09M/xKWGf0QHWkjup/LRR1FxL/e9bZSRp7L7m3NhudCW1MsHhGH8eIx/N4O9P50Yd25YB/uu7Qj1DLgtw/JVKH1sTZL9XBDyCsSpx1ei+5Oj0I8bh5o1Pyb3k/m9BPuw9qbTFLgXJwVuLiDCAfqjPWCMxVnNk71hF6ybX4aP3Jb65tmofvHdrPTxCecViM7t21A06xYoSkr57KdNb1y9kgL3wFvGKuACgjNAp21tQID93NRz5iR0dVeOVAZ6clPLKxC5GWK8FjZwb79pOn3AN3DtmgiEUq/D9H3/jBf8H28NOiDY+Ty7+dc4+sYvo1ObCMTYl16Dad5t0f7BUBmUQLATu3vBHFhaL4bnOBaIIgrQN2QSoK8xWoMWiNjAHQEiVwH6WmAyaIFgJ6tx1Qo0H2yIBushS5diZP0z12Ies7Y5qIGIBO4iuvXRqNSDLkDHojeogWAf5Iu3N6D1vd9i4nMvDroA/X8FBPsw5ze/hRErV8c+16CrD/o3YtDNOM+ArwPBMzFXm3wdiKs94zz2rgPBMzFXm3wdiKs94zz2/gsOGn1N12dXzQAAAABJRU5ErkJggg==;" vertex="1" parent="1">
          <mxGeometry x="880" y="680" width="39.2" height="40" as="geometry" />
        </mxCell>
      </root>
    </mxGraphModel>
  </diagram>
</mxfile>


==> extra.tex <==
\begin{comment}
\begin{table*}[h]
    \small
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \rowcolor{totalcolor}
        \textbf{Category} & \textbf{PG Exec Err} & \textbf{PG Reason Err} & \textbf{SG Fait Err} & \textbf{Total Examp} \\
       
        Algebra & 8 & 5 & 2 & 15 \\
        
        Prealgebra & 4 & 11 & 0 & 15 \\
     
        Probability & 8 & 6 & 1 & 15 \\
         
        Num-Theory & 6 & 7 & 3 & 16 \\
    
        Precalculus & 6 & 9 & 0 & 15 \\
    
        Int Algebra & 14 & 0 & 1 & 15 \\
      
        Geometry & 3 & 12 & 0 & 15 \\
        \rowcolor{totalcolor}
        Overall & 51 & 48 & 7 & 106 \\
        \hline
    \end{tabular}
    \caption{Summary of Error types on a Random Subset of 104 examples containing all levels of difficulty; SG Fait Err: Solution Generator changes correct output by PG to incorrect; PG Reason Err: Python code executed but had Reasoning errors, PG Exec Err: Python code by PG module had syntactical errors}
    \label{table:error_analysis}
\end{table*}
\end{comment}


\begin{comment}
\begin{figure}[!tb]
\centering
\includegraphics[width=0.7\textwidth]{images/Mathlvl_latest.png}
\caption{Accuracy vs Level of the po.}
\label{fig:pgmodule}
\end{figure}
\end{comment}



\begin{comment}
\midrule
PAS & 54.7 & 26.3& 63.5 & 30.7 & 41.6 & 44.7 & 27.3 & 43.8\\
REACT & 56.9 & 22.8 & 59.3 & 28.0 & 39.3 & 39.7 & 24.5 & 41.7 \\
REACT+PAS  & 59.6 & 26.9 & 64.0 & 30.4 & 41.6 & 43.3 & 28.6 & 45.2  \\
REACT + (\pythongenerator+\wolframalpha+\solutiongenerator)  & 61.4 & 27.1 & 63.7 & 30.7 & 40.7 & 43.0 & 30.9 & 45.9 \\
REACT + (\wolframalpha+\pythongenerator+\solutiongenerator) & 60.3 & 28.2 & 63.6 & 30.4 & 40.4 & 44.0 & 29.0 & 45.5 \\
REACT + (\bingsearch+\pythongenerator+\wolframalpha+\solutiongenerator) & 60.1 & 27.5 & 63.7 & 29.8 & 41.3 & 45.6 & 29.5 & 45.7 \\
REACT + best(by type) & 60.4 & 28.3 & 63.7 & 29.8 & 41.3 & 43.0 & 30.9 & 45.8 \\
\midrule
\end{comment}

\begin{comment}
PAS & 75.1 & 59.1 & 52.3 & 36.9 & 22.8\\
REACT & 73.2 & 56.6 & 49.4 & 35.0 & 21.4\\
REACT+PAS  &  77.2 & 60.8 & 53.6 & 37.7 & 24.2\\
REACT + (\pythongenerator+\wolframalpha + \solutiongenerator) & 78.5 &  61.1 & 53.6 & 39.0 & 25.1 \\
REACT + (\wolframalpha + \pythongenerator+\solutiongenerator) & 77.5 &  60.1 & 53.1 & 39.9 & 24.1 \\
REACT + (\bingsearch+\pythongenerator+\wolframalpha+\solutiongenerator) & 77.6 & 60.2 & 53.4 & 38.5 & 25.7 \\
REACT + best(by type) & 78.5 & 60.6 & 53.4 & 39.6 & 24.5 \\
\midrule
\end{comment}

\begin{comment}
\clearpage % Start a new page for the table
\begin{table}[htbp]
\centering

\begin{tabularx}{\textwidth}{X}
        \hline
        \textbf{[Instruction]} \newline
         Read the following question, generate the background knowledge as the context information that could be helpful for answering the question. \\ \\
         \hline
         \textbf{[Few Shot Examples]} \newline
         
         Question: Let $S$ be the set of all real numbers $alpha$ such that the function \[\frac{x^2+5x+alpha}{x^2 + 7x - 44}\] can be expressed as a quotient of two linear functions. What is the sum of the elements of $S$? \\ \\
         Mathematics Problem Type: Algebra \\ \\ 
         Level of Problem: Level 5 \\ \\ 
         Knowledge Retrieval: \\
         - The question requires using the factor and remainder theorem in Mathematics. \\
         - First factorize the denominator of the expression. \\
         - To be represented as division of linear factors, numerator should be multiple of either one of the linear factors of denominator. \\
         - Use factor theorem to get alpha for both cases and sum them to get final answer. \\ \\
         \hline
         \textbf{[Input]} \newline

         \textbf{Question}:\\ 
         New York and Denver are in different time zones.  When it is noon in New York, it is 10 a.m. in Denver.  A train leaves New York at 2 p.m. (New York time) and arrives in Denver 45 hours later.  What time is it in Denver when the train arrives? \\ \\
         \textbf{Mathematics Problem Type}:Algebra \\ \\
         \textbf{Level of Problem}:Level 3 \\ \\
         \textbf{Knowledge Retrieval}:\\ 
         - The question involves understanding of time zones and time differences between different locations.\\ 
         - The time difference between New York and Denver is 2 hours (New York is 2 hours ahead of Denver). \\ 
         - The train leaves New York at 2 p.m. New York time, which is equivalent to 12 p.m. Denver time (since Denver is 2 hours behind New York). \\ 
         - The train takes 45 hours to travel from New York to Denver. \\ 
         - To find the time in Denver when the train arrives, we need to add 45 hours to the time it left New York (2 p.m. New York time or 12 p.m. Denver time). \\ 
         - We can convert the total number of hours to the time in Denver by accounting for the 2-hour time difference between New York and Denver. \\ \\






\hline
\end{tabularx}
\caption{Knowledge Retrieval Prompt}
\end{table}
\end{comment}


\begin{comment}
\clearpage % Start a new page for the table
\begin{table}[htbp]
    \centering
 
    \begin{tabularx}{\textwidth}{X}
        \hline
        \textbf{[Instruction]} \newline 
        Read the following mathematical question and then write Python code using the Sympy library to answer the question or generate an intermediate result. \\ \\ 
        \hline
        \textbf{[Few Shot Examples]} \newline
        \textbf{Question}:\\ 
        A piece of yarn is $60$ cm long. The yarn is cut so that one piece is five times the length of the other piece. How many centimeters long is the shorter piece? \\ \\ 
        
        \textbf{Modules used till now}: [Knowledge Retrieval] \\ \\ 
        \textbf{Mathematics Problem Type}: PreAlgebra \\ \\
        \textbf{Level of Problem}: Level 2 \\ \\
        \textbf{Knowledge Retrieval}:\newline
        - The question involves a simple ratio problem, where the total length of the yarn is divided into two parts in a ratio of 5:1. \\
        - The total length of the yarn is given as 60 cm.\\
        - To find the length of the shorter piece, we need to divide the total length by the sum of the parts of the ratio (5 + 1 = 6) and then multiply by the part of the ratio that represents the shorter piece (1). \\ \\
        \textbf{Python Generator}: \\ \\
        Python Code, print answer.Also Output all the relevant objects in the intermediate steps of the python code. Make sure that the first line of the code is always 'from sympy import *' \\
        from sympy import *  \\
        x = symbols('x') \\
        eq = Eq(x + 5*x, 60) \\
        print("Equation:",eq) \\
        sol = solve(eq, x) \\
        print("Solution x:",sol) \\
        ans = sol[0] \\
        print("Shorter piece:",ans) \\ \\ 
         \hline
        \textbf{[Input]} \newline
        \textbf{Question}: Factor $-16x^4+x^2+2x+1$ into two quadratic polynomials with integer coefficients.  Submit your answer in the form $(ax^2+bx+c)(dx^2+ex+f)$, with $a<d$. \\ \\ 
        \textbf{Mathematics Problem Type}:Algebra \\ \\
        \textbf{Level of Problem} :Level 4 \\ \\ 
        \textbf{Python generator}:\\ 
        from sympy import * \\
        x = symbols('x') \\
        expr = -16*x**4 + x**2 + 2*x + 1 \\
        factors = factor(expr) \\
        print(\"Factored expression:\", factors) \\ \\
        \textbf{Python output}: \\
        Factored expression: -(4*x**2 - x - 1)*(4*x**2 + x + 1) \\
                

\hline
\end{tabularx}
\captionsetup{justification=centering}
\caption{Program Generator Prompt}
\end{table}
\end{comment}

% to perform our experiments on math related datasets.
% \textbf{MathInstruct} and \textbf{MATH} datasets.

% The overall architecture of the framework used is presented in \textcolor{blue}{Figure \ref{fig:best_setting_demonstration}}. 
% We use external tools such as the Wolfram Alpha API, Bing Web Search API, python code generators, LLM-based knowledge retrievers as parts of our compositional pipeline. 
% \textcolor{red}{Mention this details under Methodology}

% Most of our experiments use GPT-3.5-Turbo (without any finetuning) as the base LLM since it is more accessible and cheaper compared to the better performing GPT-4. We experiment with different combinations of modular settings on the data and uncover the advantages and disadvantages of each module as a function of the math problem type, the level of the problem, problem complexity. 
% Different LLMs such as CodeLlama, Llama2, etc. are also used in some ablations to explore the interactions of different LLM models. 

% \textcolor{red}{Finally, we explore two methods in planning - (1) The first one where a planner (an LLM) selects the set of modules to use based on a question and executes the sequence - which is similar to \textbf{Plan-Then-Execute} strategy, (2) A more stronger \textbf{thought-action-execution (REACT)} like setup where a central LLM generates thoughts at each step and calls any tool it requires based on that thought. Both of these experiments give us additonal insights into whether giving more power to the LLM for performing planning can improve its performance.} 
%We find that our setting with a python code generator module using the \textbf{Sympy} library and python code interpreter, used in conjuction with a downstream text-based LLM (GPT-3.5-Turbo compiling the final steps in the solution) achieves an overall performance of 46.2 percent on the MATH dataset which is a \textcolor{blue}{5.6 percent} improvement over previous state of the art  (Skills-In-Context prompting SkiC\cite{chen2023skillsincontext}). 

%Our experiments with ChatGPT as a knowledge retriever and search engine-based retrievers like Bing Web Search API show that Bing search can outperform the former through the extraction of highly relevant snippets from the web that are most similar to the question and extraction of relevant knowledge such as formulas or concepts related to the question. Contrary to this, we find that LLM generated knowledge or hints to solve a problem can be very vague or often misleading that can push the downstream modules on an incorrect solution path. In fact, LLM-based knowledge retrievers add very little compared to simple Chain of Thought prompting techniques.

%We also find from our experiments that WolframAlpha alone used in conjuction with a dowmstream text-LLM can match our python code-based setting closely, even outperforming it on certain types of mathematical problems like \textbf{Intermediate Algebra}. This setting has a accuracy of \textcolor{blue}{30.45 percent} on Intermediate Algebra - the toughest problem type on MATH which is a \textcolor{blue}{12.4 percent} increase over SkiC and a \textcolor{blue}{9.3 percent} increase over our Python setting. This clearly shows how grounding queries in symbolic languages (here Wolfram language) can help solve more difficult problems in certain math subdomains. In addition, combining both Wolfram Alpha modules and python code based modules further improves the overall performance compared to using each module separately, clearly showing the advantages associated with intelligent combination of modules through a planning process. Along this direction, our experiments with SOTA planning techniques show that ....

%In summary, our contributions are as follows:\\ \\ \textbf{(1)} We evaluate the performance of tool-augmented LLMs on math reasoning using different combinations of modules meticulously quantifiying the advantages and disadvantanges of each module as a function of dataset, the subdomain in mathematics (Algebra, Calculus, etc.), problem level (0-5) and the complexity of the problem. Our best setting outperforms previous state-of-the-art techniques to solve the MATH dataset using GPT-3.5-Turbo by a significant margin.\\ \\
%The best setting from our experiments achieves a performance accuracy of - on the MATH dataset outperforming previous baseline techniques using GPT-3.5-Turbo. %Our paper helps uncover some interesting patterns and observations in relation to tool-augmented LLMs in mathematical reasoning. These insights can be extremely useful to overcome some of the aforementioned limitations that compositional methods in MATH presently have. Our experiments share some exciting findings:-  
%\textbf{(1)} Our setting with a python code generator module using the \textbf{Sympy} library and python code executor, used in conjuction with a solution generator module (LLM)  achieves the best overall performance of 46.2 percent on the MATH dataset which is a \textbf{4.2 percent} performance increase over GPT4 with CoT, \\ \\ \textbf{(2)} Our experiments with the \textbf{Wolfram Alpha API} show that using simply the Wolfram-Alpha module used in conjuction with a solution generator module (LLM) outperforms the performance of the python setting on certain mathematical problems like \textbf{Intermediate Algebra}. Our Wolfram Alpha setting has a accuracy of 30.45 percent on Intermediate Algebra - the toughest problem type on MATH which is a 9.3 percent increase (21.1 percent) over the Python setting. This clearly shows that Wolfram Alpha can indeed compare with and outperform python code representations and thus it is necessary to explore ways of integrating the two in an optimal way to get the best out of both.\\ \\ 
%\textbf{(3)} Our experiments with the \textbf{knowledge retrieval} module shows that adding background knowledge/hints/plans to solve a problem before the solution generator module does not improve the performance of the setting. In fact, we use weaker models like \textbf{text-davinci-002, text-davinci-003, Llama2-7B} as the knowledge retrieval module to show that the reduction in the quality of knowledge or information added can detoriate the performance of the GPT-3.5-Turbo based solution generator module (which is similar to CoT). \\ \\
%\textbf{(4)} We find through the comparison of different planning strategies that the \textbf{REACT-like setting} which gives the highest degree of power to the LLM for using any tool it wants (with precise rationales of what it needs) outperforms other methods which fix the sequence of modules before starting run on an example, clearly constraining the planning power of the system.
%Mathematical reasoning has been an important dimension to test LLMs, since it is an important aspect of human intelligence and logic, and has applications in various other fields of study. While LLMs have shown significant improvements in performance in simple mathematical datasets like GSM-8K \cite{cobbe2021gsm8k}, there is still a significant gap from human-level performance on complex mathematics tasks datasets like MATH \cite{ hendrycks2021measuring}. For example, GPT-4 shows poor performance on the MATH dataset with a 42 percent accuracy, and in addition, there is a large cost associated with running these commercial models. This motivates our study on compositional methods using modular architectures, comprising GPT-3.5-Turbo and other open-source models like CodeLlama, Llama2, etc on the task of mathematical reasoning. \\ 
%\noindent LLMs can suffer from limitations like generating unfactual information which are unverifiable but seemingly plausible, a phenomenon called hallucinations in LLMs \cite{tam2022evaluating,sun2023head}. This can result in errors in the reasoning chains or incorrect assumptions in the outputs that may be possible to avoid. Motivated by the need to tackle this issue, there has been a recent increasing trend towards augmenting tools and libraries with language models, a paradigm referred to as Augmented Language Models (ALMs) \cite{mialon2023augmented}. These tool-augmented LLMs have the advantages of calling external modules like API's, python code generators, libraries or web search engines which can help retrive factual information, and take advantage of the strengths of these modules. Often such setups are compositional in nature, where the outputs or the information from previous modules is utilized as context for downstream modules. Recent works such as Chameleon \cite{lu2023chameleon} has deployed such methods for tasks like ScienceQA \cite{lu2022learn}, TabMWP \cite{lu2023dynamic}, etc. but have not been evaluated on more complex mathematical reasoning datasets like MATH. Similarly, the framework ART  \cite{paranjape2023art} looks at integrations of tools with limited supervision, and performs evaluation on tasks from BigBench, MMLU, as well as datasets like SQUAD, TriviaQA, SVAMP, MAWPS, etc. While these papers look at some LLMs as component models, there has not been a more detailed study of how different modules interact when different LLMs are used as their base models. For example, there are a number of models like Codex, CodeLlama, CodeLlama-Python, etc. which are viable choices for code generation models. Similarly, there can be various base models like Llama2, Text-davinci, GPT-3.5-Turbo that can be used for knowledge retrieval modules. The question here is which models when used in combination can produce the most optimal results. Another caveat is the order of execution of the modules to be used, depending on the features of the problem at hand. With regard to this, there are two possibilities - one to use setup where the central LLM calls the tools when it requires and performs some action using these tools. The other possibility is to have a dynamic planner that can output the sequence of modules to be executed using the features of the problem such as level of problem, subdomain of mathematics involved, skills required, complexity, etc. \\   
% To tackle these issues and investigate the complexities involved,we perform an in-depth analysis on the combinations of different modules, some of them using base LLMs and open-source models. We also look at external tools like Wolfram Alpha API, Bing Search, etc. and quantify the advantages/disadvantages of using these tools on different types of math problems. We also observe that some mathematical problems may favour solutions in code representations while some may perform better with natural language representations. Some of the problems may benefit from a combination of the two, by utilizing the best of both worlds. We investigate these situations, through different module combinations. We perform an in-depth analysis into the type of errors that our best modular setting makes on different types of problems and discover certain mathematical concepts that the pipeline fails to understand. To confirm our findings, we probe a single GPT-3.5-Turbo instance on these sensitive points and find some absurd mistakes that the model makes. In addition, we also perform analysis with respect to the relationships between the complexity of the problem and the accuracy of different settings. In order to do this, we use complexity measures from code forms like abstract syntax trees (AST) such as number of function calls, variable names, mathematical operations, etc. We also use complexity measures derived from text forms, such as number of intermediate steps to gain additional insights into this dimension.
%The ability of languagtures if e models to performing reasoning is an important goal to achieve. While, LLMs seem to be getting better on simple reasoning datasets, they seem to fail when dealing with more complex reasoning operations. Failure is mainly of two types: one where models fail to ground the generations in the context and hallucinate unverifiable content(unfactual). The second type is one where the model makes a logical/reasoning error in their output generations.While approaches centered around Chain Of Thought (Nye et al.,2021; Wei et al.,2022; Kojima et al.,2022) use step-by-step explanations to generate the reasoning steps, there has been related research on the unreliability of these explanations in in-context learning(Ye and Durrett, 2022) which has shown that simply adding explanations to prompts does not always improve performance of these models. Other work (Ling and Fang, 2023) has looked at the use of deductive reasoning through self verification to alleviate the problems of grounding and logical errors. However, their work does not completely eliminate this phenomenon and LLMs can still produce harmful and biased content, make incorrect claims, and produce wrongful advice particularly in more complex and longer reasoning chains. 
%There has been a growing interest in the use of symbolic grammars in place of natural language representations to represent problems in LLMs. LOGIC-LM() looks at one such approach on datasets of deductive reasoning, first order logic and constraint satisfaction problems. Here, LLMs instead of solving the entire problem, are only used for the conversion of natural language to symbolic grammars involving predicate logic, FOL(First order logic) representations and the main task of solving is left to domain-specific solvers. (Gao Madan Zhou 2023;) uses code-representations in python as intermediate reasoning steps and offloads the final calculation to an interpreter. This synergy between the LLM and python interpretor produces very promising results for them on state-of-the-art reasoning tasks like BigBench Hard. Through our work, we aim to take this idea one step forward by using pseudo-code representations(a mix of language and latex format pseudo-code) and having LLM agents debate in this symbolic code language. The idea is to have agents figure out errors like grounding, calculation or logical on their own through a collaborative environment of discussion and deliberation. Based on the debate arguments, an expert provides the agents with feedback to improve upon their answers.
%We maintain the advantages of modularity as in works like LOGIC-LM as well combine it with the power of debate as seen in recent works like (). We also use the pseudo-code of each agent to generate an executable python code to get the final answer, which brings down the errors related to the  unfaithfulness of the final answer to explanations. We aim to facilitate the debate by providing short feedback in terms of line numbers of logically incorrect code, important debate points,etc instead of long explanations. Our hope is that by providing more attention to these parts of the pseudo-code the model will learn to figure out the issues on its own. We conduct studies to evaluate the performance of different models in this debate setup (both agents same model/ different) with a special focus on models trained on code like code-davinci, phi, etc. Since studies have shown that models trained on code have greater symbol-binding capabilities this is also natural and backed by observations.
%\vspace{2mm}
%\textcolor{red}{Pre-trained Large Language Models (LLMs) have shown remarkable performance on a wide variety of NLP tasks} \textcolor{blue}{[Rephrase the previous text]} using strategies like Chain of Thought and Program of Thought prompting. \textcolor{red}{They} \textcolor{blue}{[Be more specific about which method you are referring to. Avoid usage of 'They', 'It', etc. (as much as possible)]} have demonstrated abilities to generalize to a new task through in-context learning \textcolor{blue}{[give some background about in-context learning, zero-shot and few-shot learning before referring such methods]} by simply utilizing few-shot examples in the prompt \textcolor{blue}{[explain what do mean by prompt?]}. In addition, there has also been a rise of \textcolor{red}{compositional methods} through the integration of modules and tools with these LLMs \textcolor{blue}{['these LLMs'? Briefly explain the concept of compositional method, and how LLMs are being used for performing different tasks, then provide examples, e.g., Chameleon, Toolformers, etc.]} as seen in recent works (Chameleon, Toolformers, etc.) \textcolor{blue}{[Cite the papers of chameleon and toolformers]}. Although, such strategies of integration have shown significant improvements in state-of-the-art performance for several knowledge intensive reasoning tasks like \textcolor{red}{question answering, simple math word problems} \textcolor{blue}{[try to be more specific, provide citations of existing datasets]}, etc., there has been little analysis on \textcolor{red}{\textit{i) how these tools interact with one another}, \textit{ii) what is the relationship between the modules}, \textit{iii) which subset of modules are apt at solving specific problems}, iv) \textit{what should be the optimal policy for execution of the modules}}\textcolor{blue}{[need to rephrase, try to use either 'tools' or 'modules', better not to confuse the reader by using them interchangeably]}.
%In this paper, we focus on analysing \textcolor{red}{these effects} \textcolor{blue}{what effects?} on mathematical datasets like MATH \textcolor{blue}{[provide citation of MATH dataset; mention other datasets]} which require complex reasoning. We \textcolor{red}{construct a pipeline consisting of modules for python code generation, knowledge retrieval, Wolfram Alpha calls, solution generator} \textcolor{blue}{[try to portray an abstract view of our approach; rephrase]}, etc for this task. 
%In this work , we concentrate primarily on this paradigm of tool-augmented language models \cite{mialon2023augmented} in the context of complex mathematical reasoning.

%Recent works on this paradigm such as  Chameleon \cite{lu2023chameleon} augments LLMs with  plug-and-play modules for compositional reasoning to solve knowledge intensive reasoning datasets like ScienceQA \cite{lu2022learn}, TabMWP \cite{lu2023dynamic}. Another work OlaGPT \cite{xie2023olagpt} develops a cognitive architecture framework with tools, and simulates certain aspects of human cognition by incorporating different cognitive modules, including attention, memory, reasoning, learning, and corresponding scheduling and decision-making mechanisms. Similarly, the framework ART  \cite{paranjape2023art} looks at integrations of tools with limited supervision, and performs evaluation on tasks from BigBench, MMLU. 

%\textit{Are there specific modules that work best on certain problem types? Are all modules used in such pipelines equally useful? } We discuss the complimentary abilities that such tools and APIs can bring about when integrated with LLMs. We analyze these effects in the domain of mathematical reasoning using the \textbf{MATH} and the newly released \textbf{MathInstruct} dataset which we select owing to its diversity in math problem type and tasks.
%In this work , we concentrate primarily on this paradigm of tool-augmented language models \cite{mialon2023augmented} in the context of complex mathematical reasoning.
%There has also been little comparison of symbolic tools like code-generators, knowledge retrievers like search engines with LLM-based tools - as a function of the mathematics problem type such as algebra, geometry, calculus, etc. External API's like Wolfram Alpha are known to hold large volumes of math knowledge, but do these tools actually contribute complementary information compared to LLMs. How do their contributions vary as a function of the level of difficulty. There are further questions as to which planning methods are suitable for such tool-augmented frameworks and whether we can intelligently select tools for simpler problems and achieve an improvement on performance.    

%Recently, there has been much progress with the introduction of various tool-augmented frameworks such as Chameleon, OlaGPT, ART and SocraticAI.

%Mathematical reasoning is an important dimension which can serve as a measure of the intelligence and logical capabilities of LLMs. While performing well on simple high school math datasets like GSM-8k, they falter at more complex mathematics of higher difficulty. As a result, we focus on datasets like MATH and MathInstruct, which have a collection of diverse problem types and tasks. Specifically, we investigate the following: 
%(1) Do pipelines with code modules outperform those with text modules across all types of mathematics datasets or do simpler problems favour the latter? Additionally, is there a certain trend between the complexity of generated python code and their solution accuracy? 
%(2) Do knowledge bases like Wolfram-Alpha and LLM-based knowledge retrievers improve the problem solving abilities and if so specifically in which type of mathematics problem ?
%(3) Is there an optimal combination of modules or an ensemble which achieves the best performance across all math reasoning tasks? 
%(4) Do planning methods improve the reasoning capabilities of augmented LLMs and how do the state-of-the-art planning methods compare against each other?

%Motivated by the need to tackle this issue, there has been a recent increasing trend towards augmenting tools and libraries with language models, a paradigm referred to as Augmented Language Models (ALMs) \cite{mialon2023augmented}. 

%Such modular architectures can help take advantage of the unique and complementary set of skills in each tool, and improve the performance of the foundation LLM. Recent works such as Chameleon \cite{lu2023chameleon} and MMREACT \cite{yang2023mm} have deployed such methods for multi-modal knowledge intensive tasks like ScienceQA \cite{lu2022learn}, TabMWP \cite{lu2023dynamic}, etc. Similarly, the framework ART  \cite{paranjape2023art} looks at integrations of tools with limited supervision, and performs evaluation on tasks from BigBench, MMLU, as well as datasets like SQUAD, TriviaQA, SVAMP, and MAWPS. Though LLMs do well on simple mathematical datasets like GSM-8K, there has been little focus and analysis of compositional models on complex mathematical datasets like MATH, on which commercial models like GPT-4, GPT-3.5-Turbo perform extremely poorly, even using Chain-of-Thought prompting. \textit{In addition, the existing approaches do not delve deep into how the different combinations of modules interact. Can we attribute the increase or decrease in performace to a specific module? Is there optimal combination of modules that is more suited for a particular type of problem?} It is also not clear from the existing literature whether external API's integrated with LLMs do actually contribute or add some value to the base LLM. There is also an important open question related to which kind of representations are more suited for a problem. While, overall it is true that Python code generation with interpreters have improved performance on a wide range of math datasets, there is still less exploration on the hypothesis that simpler problems might favour natural language representations. For example, a problem in Geometry may be not be inherently well suited for Python without multi-modal capabilities because of the lack of useful geometry libraries. Finally, it is also important to quantify if giving the power to use tools to a central LLM using thought, action- observation like setups inspired from \cite{yao2022react}, can outperform methods, which fix a sequence of tools to be executed beforehand on a per example basis. \\


"problem": "If the fourth term of an arithmetic sequence is $200$ and the eighth term is $500$, what is the sixth term?",


"response": "Mathematics Problem Type:Algebra\nLevel of Problem:Level 1\n\n


, 
(SIMILAR QUESTIONS)


"bing_query1": "If the fourth term of an arithmetic sequence is $200$ and the eighth term is $500$, what is the sixth term?\n\n", 


OUTPUT:
Question 1:Find the 16th term of arithmetic sequence with common difference 2? 
From the given, a 1 = 0 ; n = 16 ; d = 2 a 16 = 0 + (16 - 1)2 a  = 15 * 2 = 30 


Question 2: Find the sum of the first 30 terms of the following sequence. 4, 7, 10, 13,\u2026. 
Solution: The given arithmetic sequence is: 4, 7, 10, 13,\u2026. Here,", "There are formulae introduced that can help in finding the value with limited given options, for instance, finding the n th term from first and the last term only. Let\u2019s say a series A consist of some element a 1, a 2, a 3, a 4, a 5, a 6 ,\u2026an A = {a 1, a 2, a 3, a 4, a 5, a 6 ,\u2026 a n } Common difference between two terms (d) = (a1-a2)"], 


Examples : Identify the Sequence Find the Next Term Popular Problems Identify the Sequence 4,12,36,108 4, 12, 36, 108 Identify the Sequence 3,15,75,375 3, 15, 75, 375",






bing_query2": " What is the formula for the nth term of an arithmetic sequence?"


Concepts search output: ["The main difference between sequence and series is that, by definition, an arithmetic sequence is simply the set of numbers created by adding the common difference each time. 


Arithmetic series, on the other head, is the sum of n terms of a sequence. For example, you might denote the sum of the first 12 terms with S12 = a1 + a2 + ... + a12.", 


It is represented by the formula a_n = a_1 + (n-1)d, where a_1 is the first term of the sequence, a_n is the nth term of the sequence, and d is the common difference, which is obtained by subtracting the previous term from the current term. How do you know if a sequence is arithmetic or geometric?"],
FINAL EXTRACTED OUTPUT (MAY NOT SHOW IN FIGURE IF IT DOESN'T FIT)
"bing_search:output": "The formula for a_n in an arithmetic sequence is a_1 + (n-1)d, where a_1 is the first term of the sequence, a_n is the nth term of the sequence, and d is the common difference, which is obtained by subtracting the previous term from the current term.\nThe nth term formula for an arithmetic sequence is: an = a1 + (n-1)d, where a1 is the first term, d is the common difference, and n is the term number. This formula can be used to find the sixth term if the fourth and eighth terms are known."

\begin{comment}
BING-SG - 427 EXAMPLES
PG-BING-SG - 339 EXAMPLES
BING-PG-WALPHA-SG - 196 EXAMPLES
BING-PG-SG : 304 EXAMPLES
\end{comment}
